Generative Lines Matching Models

In this paper we identify the source of a singularity in the training loss of key denoising models, that causes the denoiser's predictions to collapse towards the mean of the source or target distributions. This degeneracy creates false basins of attraction, distorting the denoising trajectories and ultimately increasing the number of steps required to sample these models. We circumvent this artifact by leveraging the deterministic ODE-based samplers, offered by certain denoising diffusion and score-matching models, which establish a well-defined change-of-variables between the source and target distributions. Given this correspondence, we propose a new probability flow model, the Lines Matching Model (LMM), which matches globally straight lines interpolating the two distributions. We demonstrate that the flow fields produced by the LMM exhibit notable temporal consistency, resulting in trajectories with excellent straightness scores. Beyond its sampling efficiency, the LMM formulation allows us to enhance the fidelity of the generated samples by integrating domain-specific reconstruction and adversarial losses, and by optimizing its training for the sampling procedure used. Overall, the LMM achieves state-of-the-art FID scores with minimal NFEs on established benchmark datasets: 1.57/1.39 (NFE=1/2) on CIFAR-10, 1.47/1.17 on ImageNet 64x64, and 2.68/1.54 on AFHQ 64x64. Finally, we provide a theoretical analysis showing that the use of optimal transport to relate the two distributions suffers from a curse of dimensionality, where the pairing set size (mini-batch) must scale exponentially with the signal dimension.

==> draft.tex <==
title "conditional latent distributions for generative modeling"

[classifier-free], Conditional denoising models are primarily trained to transform general noise distributions into the conditioned target data. The conditioning variable is typically encoded and spread across the network architecture to effectively influence its behavior. Consequently, in this paradigm the entire latent distribution is mapped to every conditioned mode in the target distribution. Recent works~[poodlian23 and Tong24] show that by increasing the specificity and minimizing the distance between latent variables and data samples during training, straighter probability flows are produced and fewer sampling steps are needed at inference time. This is in comparison to the non-specific random pairing between the distributions typically used for training denoising-based models.
 
In this work we leverage the availability of the conditioning variable to achieve this goal, namely, infer a non-trivial and close association between the latent and the target data distributions. However, rather than solving pairing problems with non-linear complexity we shape the latent distribution to align more closely with the data. Specifically, we construct a Conditional Latent Distribution (CLD) using a Gaussian Mixture Model (GMM), where each conditioning state, such as a label, is represented by a Gaussian fitted to the data samples corresponding to that state.

As illustrated in Figure 1, when mapping a generic latent distribution to a specific mode in the data that occupies a small fraction of the target distribution, latent and data points that are far apart must be associated with high noise levels during training. Similarly, very long trajectories must be followed during sampling due to these remote pairings. By contrast, the CLD restricts the latent regions associated with each data mode, and induces a narrower joint distribution, containing lower noise levels, over latent and target variables. Moreover, the CLD gives rise to sampling trajectories already start in the approximated target mode and has a lesser distance to follow. [and hence can be viewed as the final sengments of the trajectories produced in the generic case ]

. Our experiments shows that using the CLD and the joint distribution it induces leads to significant gains both in training and sampling efficiency.
 v


==> prev.tex <==
\section{Previous Work}
\label{sec:prev}


==> tables_chat.tex <==
\begin{table}
\centering
\tiny
\setlength{\tabcolsep}{3pt}

\begin{subtable}[t]{0.48\textwidth}
\centering
\caption{CIFAR-10}
\label{tab:cifar}
\begin{tabular}{@{}l c c c c@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\textbf{NFE}} & \multicolumn{2}{c}{\textbf{Unconditional}} & \multicolumn{1}{c}{\textbf{Conditional}}\\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-5}
& & FID & IS & FID \\ \midrule
\textbf{GAN} \\
BigGAN~\cite{biggan} & 1 & 14.70 & 9.22 & - \\
StyleGAN2-ADA~\cite{StyleGANADA} & 1 & 2.92 & 9.83 & 2.42 \\
StyleGAN-D2D~\cite{StyleGAND2D} & 1 & - & - & 2.26 \\
StyleGAN-XL~\cite{Sauer2022StyleGAN} & 1 & - & - & 1.85 \\ \midrule
\textbf{Diffusion / Score Matching} \\
DDPM~\cite{Ho2020DDPM} & 1000 & 3.17 & 9.46 & - \\
DDIM~\cite{Song2021implicit} & 100 & 4.16 & - & - \\ 
Score SDE~\cite{Song2021SMLD} & 2000 & 2.20 & 9.89 & - \\ 
EDM~\cite{Tero2022EDM} & 35 & 1.97 & 9.84 & 1.79  \\ \midrule
\textbf{Distillation / Direct Gen.} \\
KD~\cite{Luhman2021knowdistl} & 1 & 9.36 & 8.36 & - \\
PD~\cite{Salimans2022PD} & 1 & 9.12 & - & - \\
CT~\cite{Song23CM} & 1 & 8.70 & 8.49 & - \\
CD~\cite{Song23CM} & 1 & 3.55 & 9.48 & - \\
CD+GAN~\cite{Lu2023CMGAN} & 1 & 2.65 & - & - \\
iCT~\cite{song2024improved} & 1 & 2.83 & 9.54 & - \\
iCT-deep~\cite{song2024improved} & 1 & 2.51 & 9.76 & - \\
CTM~\cite{Kim2024CTM} & 1 & 1.98 & - & 1.73 \\
DMD~\cite{yin2024onestepdmd} & 1 & 3.77 & - & 2.66 \\
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & 2.02 & 10.02 & 1.93 \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.92 & 9.98 & 1.71 \\
PD~\cite{Salimans2022PD} & 2 & 4.51 & - & - \\
CT~\cite{Song23CM} & 2 & 5.83 & 8.85 & - \\
CD~\cite{Song23CM} & 2 & 2.93 & 9.75 & - \\
iCT~\cite{song2024improved} & 2 & 2.46 & 9.80 & - \\
iCT-deep~\cite{song2024improved} & 2 & 2.24 & 9.89 & - \\
CTM~\cite{Kim2024CTM} & 2 & 1.87 & - & 1.63 \\ \midrule
\textbf{Flow Matching} \\
OT-CFM~\cite{Lipman2023flow} & 142 & 6.35 & - & - \\
1-Rect-Flow (distill)~\cite{Liu2023RectFlow} & 1 & 6.18 & 9.08 & - \\
2-Rect-Flow (distill)~\cite{Liu2023RectFlow} & 1 & 4.85 & 9.01 & - \\
3-Rect-Flow (distill)~\cite{Liu2023RectFlow} & 1 & 5.21 & 8.79 & - \\
1-Rect-Flow~\cite{Liu2023RectFlow} & 127 & 2.58 & 9.60 & - \\
2-Rect-Flow~\cite{Liu2023RectFlow} & 110 & 3.36 & 9.24 & - \\
2-Rect-Flow~\cite{Liu2023RectFlow} & 104 & 3.96 & 9.01 & - \\ \midrule
LMM  & 1 & \textbf{1.90} & 10.16 & \textbf{1.57}\normalfont \\
LMM  & 2 & \textbf{1.55} & 10.20 & \textbf{1.39}\normalfont \\ \bottomrule
\end{tabular}



\begin{tabular}{c}
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{ccccc}
         \multirow{2}{*}{\textbf{EDM}} & \multicolumn{4}{c}{\textbf{LMM}} \\\cmidrule(lr){2-5} 
            & \multicolumn{2}{c}{ wo/ADL} & \multicolumn{2}{c}{ w/ADL} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
         NFE 79 & NFE 1 & NFE 2 & NFE 1 & NFE 2 \\
    \end{tabular} \vspace{0.02in} \\
    \includegraphics[width=2.3in]{figs/results/comparison.png}
    \end{tabular}
    
    \caption{ImageNet \rsm~Samples Comparison.}
    \label{tab:visual}

    
\end{subtable}
\hfill
\begin{subtable}[t]{0.48\textwidth}
\centering
\caption{ImageNet \rsm}
\label{tab:imagenet}
\begin{tabular}{@{}l c c c@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\textbf{NFE}} & \multicolumn{2}{c}{\textbf{Conditional}} \\ \cmidrule(lr){3-4}
& & \textbf{FID} & \textbf{IS} \\ \midrule
\textbf{GANs} \\
BigGAN-deep~\cite{biggan} & 1 & 4.06 & - \\
StyleGAN-XL~\cite{Sauer2022StyleGAN} & 1 & 1.51 & 82.35 (?) \\ \midrule
\textbf{Diffusion / Score Matching} \\
RIN~\cite{Jabri23RIN} & 1000 & 1.23 & - \\
EDM~\cite{Tero2022EDM} & 511 & 1.36 & - \\
DDPM~\cite{Ho2020DDPM} & 250 & 11 & - \\
EDM~\cite{Tero2022EDM} & 79 & 2.23 & 48.88 (?) \\ \midrule
\textbf{Distillation / Direct Gen.} \\
PD~\cite{Salimans2022PD} & 1 & 15.39 & - \\
BOOT~\cite{gu2023boot} & 1 & 16.30 & - \\
CT~\cite{Song23CM} & 1 & 13.0 & - \\
CD~\cite{Song23CM} & 1 & 6.20 & 40.08 (?) \\
iCT~\cite{song2024improved} & 1 & 4.02 & - \\
iCT-deep~\cite{song2024improved} & 1 & 3.25 & - \\
CTM~\cite{Kim2024CTM} & 1 & 1.92 & 70.38 \\
DMD~\cite{yin2024onestepdmd} & 1 & 2.62 & - \\
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & 2.02 & - \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.52 & - \\
PD~\cite{Salimans2022PD} & 2 & 8.95 & - \\
CT~\cite{Song23CM} & 2 & 11.1 & - \\
CD~\cite{Song23CM} & 2 & 4.70 & - \\
iCT~\cite{song2024improved} & 2 & 3.20 & - \\
iCT-deep~\cite{song2024improved} & 2 & 2.77 & - \\
CTM~\cite{Kim2024CTM} & 2 & 1.73 & 64.29 \\ \midrule
\textbf{Flow Matching} \\
OT-CFM~\cite{Lipman2023flow} & 138 & 14.45 & - \\
BOT-CFM~\cite{Pooladian2023mini} & 132 & 11.82 & - \\ \midrule
LMM & 1 & \textbf{1.47} & 59.86 \\ 
LMM & 2 & \textbf{1.17} & 61.18 \\ 
\bottomrule
\end{tabular}
\end{subtable}

\vspace{0.3cm}

\begin{subtable}[t]{0.48\textwidth}
\centering
\caption{AFHQ \rsm}
\label{tab:afhq}
\begin{tabular}{@{}l c c@{}}
\toprule
Model & \textbf{NFE} & \textbf{FID}\\ \midrule
\textbf{Score Matching} \\
EDM~\cite{Tero2022EDM} & 79  & 1.96 \\ \midrule
\textbf{Distillation} \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.71  \\ 
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & \textbf{1.63}  \\ \midrule
LMM & 1  &  2.68 \\
LMM & 2  &  \textbf{1.54}  \\ \bottomrule
\end{tabular}
\end{subtable}

\normalsize
\end{table}

==> tables_tmp2.tex <==
\begin{table}
\vspace{-0.07in}
\centering
\renewcommand{\arraystretch}{1.0} % Adjust row separation
\tiny % Reduced font size
\setlength{\tabcolsep}{3pt} % Further reduced column separation
\begin{minipage}[t]{0.48\textwidth} % Reduced minipage width
\centering
\caption{CIFAR-10}
\label{tab:cifar}
\begin{tabular}{@{}l c c c c@{}}
%\multicolumn{6}{c}{\textbf{CIFAR10}} \\
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\textbf{NFE}} & \multicolumn{2}{c}{\textbf{Unconditional}} & \multicolumn{1}{c}{\textbf{Conditional}}\\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-5}
& & FID & IS & FID \\ \midrule
\textbf{GAN} \\
BigGAN~\cite{biggan} & 1 & 8.51 & - & - \\
StyleGAN2-ADA~\cite{StyleGANADA} & 1 & 2.92 & - & 2.42 \\
StyleGAN-D2D~\cite{StyleGAND2D} & 1 & - & - & 2.26 \\
StyleGAN-XL~\cite{Sauer2022StyleGAN} & 1 & - & - & 1.85 \\ \midrule
\textbf{Diffusion / Score Matching} \\
DDPM~\cite{Ho2020DDPM} & 1000 & 3.17 & - & - \\
DDIM~\cite{Song2021implicit} & 100 & 4.16 & - & - \\ 
Score SDE~\cite{Song2021SMLD} & 2000 & 2.20 & - & - \\ 
EDM~\cite{Tero2022EDM} & 35 & 1.97 & - & 1.79  \\ \midrule
\textbf{Distillation / Direct Gen.} \\
KD~\cite{Luhman2021knowdistl} & 1 & 9.36 & - & - \\
PD~\cite{Salimans2022PD} & 1 & 9.12 & - & - \\
CT~\cite{Song23CM} & 1 & 8.7 & - & - \\
CD~\cite{Song23CM} & 1 & 3.55 & - & - \\
CD+GAN~\cite{Lu2023CMGAN} & 1 & 2.65 & - & - \\
iCT~\cite{song2024improved} & 1 & 2.83 & - & - \\
iCT-deep~\cite{song2024improved} & 1 & 2.51 & - & - \\
CTM~\cite{Kim2024CTM} & 1 & 1.98 & - & 1.73 \\
DMD~\cite{yin2024onestepdmd} & 1 & 3.77 & - & 2.66 \\
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & 2.02 & - & 1.93 \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.92 & - & 1.71 \\
PD~\cite{Salimans2022PD} & 2 & 4.51 & - & - \\
CT~\cite{Song23CM} & 2 & 5.83 & - & - \\
CD~\cite{Song23CM} & 2 & 2.93 & - & - \\
iCT~\cite{song2024improved} & 2 & 2.46 & - & - \\
iCT-deep~\cite{song2024improved} & 2 & 2.24 & - & - \\
CTM~\cite{Kim2024CTM} & 2 & 1.87 & - & 1.63 \\ \midrule
\textbf{Flow Matching} \\
OT-CFM~\cite{Lipman2023flow} & 142 & 6.35 & - & - \\
2-Rect-Flow (distill)~\cite{Liu2023RectFlow} & 1 & 4.85 & - & - \\
1-Rect-Flow~\cite{Liu2023RectFlow} & 127 & 2.58 & - & - \\ \midrule
LMM  & 1 & \textbf{1.90} & - & \textbf{1.57}\normalfont \\
LMM  & 2 & \textbf{1.55} & - & \textbf{1.39}\normalfont \\ \bottomrule  \vspace{0.05in}
\end{tabular}

\begin{tabular}{c}
    \setlength{\tabcolsep}{6pt} % Slightly increased for clarity
    \begin{tabular}{ccccc}
         \multirow{2}{*}{\textbf{EDM}} & \multicolumn{4}{c}{\textbf{LMM}} \\\cmidrule(lr){2-5} 
            & \multicolumn{2}{c}{wo/ADL} & \multicolumn{2}{c}{w/ADL} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
         NFE 79 & NFE 1 & NFE 2 & NFE 1 & NFE 2 \\
    \end{tabular} \vspace{0.02in} \\
    \includegraphics[width=2.3in]{figs/results/comparison.png}
\end{tabular}
    
\caption{ImageNet \rsm~Samples Comparison.}
\label{tab:visual}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth} % Adjusted minipage width
\centering
\caption{ImageNet \rsm}
\label{tab:imagenet}
\begin{tabular}{@{}l c c c@{}}
%\multicolumn{4}{c}{\textbf{ImageNet64}} \\
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\textbf{NFE}} & \multicolumn{2}{c}{\textbf{Conditional}} \\ \cmidrule(l){3-4}
& & \textbf{FID} & \textbf{IS} \\ \midrule
\textbf{GANs} \\
BigGAN-deep~\cite{biggan} & 1 & 4.06 & - \\
StyleGAN-XL~\cite{Sauer2022StyleGAN} & 1 & 1.51 & 82.35 (?) \\ \midrule
\textbf{Diffusion / Score Matching} \\
RIN~\cite{Jabri23RIN} & 1000 & 1.23 & - \\
EDM~\cite{Tero2022EDM} & 511 & 1.36 & - \\
DDPM~\cite{Ho2020DDPM} & 250 & 11 & - \\
EDM~\cite{Tero2022EDM} & 79 & 2.23 & 48.88 (?) \\ \midrule
\textbf{Distillation / Direct Gen.} \\
PD~\cite{Salimans2022PD} & 1 & 15.39 & - \\
BOOT~\cite{gu2023boot} & 1 & 16.30 & - \\
CT~\cite{Song23CM} & 1 & 13.0 & - \\
CD~\cite{Song23CM} & 1 & 6.20 & 40.08 (?) \\
iCT~\cite{song2024improved} & 1 & 4.02 & - \\
iCT-deep~\cite{song2024improved} & 1 & 3.25 & - \\
CTM~\cite{Kim2024CTM} & 1 & 1.92 & 70.38 \\
DMD~\cite{yin2024onestepdmd} & 1 & 2.62 & - \\
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & 2.02 & - \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.52 & - \\
PD~\cite{Salimans2022PD} & 2 & 8.95 & - \\
CT~\cite{Song23CM} & 2 & 11.1 & - \\
CD~\cite{Song23CM} & 2 & 4.70 & - \\
iCT~\cite{song2024improved} & 2 & 3.20 & - \\
iCT-deep~\cite{song2024improved} & 2 & 2.77 & - \\
CTM~\cite{Kim2024CTM} & 2 & 1.73 & 64.29 \\ \midrule
\textbf{Flow Matching} \\
OT-CFM~\cite{Lipman2023flow} & 138 & 14.45 & - \\
BOT-CFM~\cite{Pooladian2023mini} & 132 & 11.82 & - \\ \midrule
LMM & 1 & \textbf{1.47} & - \\ 
LMM & 2 & \textbf{1.17} & - \\ 
\bottomrule
\end{tabular}

\vspace{0.3cm} % Reduced vertical space

\caption{AFHQ \rsm}
\label{tab:afhq}
\begin{tabular}{@{}l c c@{}}
%\multicolumn{4}{c}{\textbf{AFHQ64}} \\ 
\toprule
Model & \textbf{NFE} & \textbf{FID}\\ \midrule
\textbf{Score Matching} \\
EDM~\cite{Tero2022EDM} & 79  & 1.96 \\ \midrule
\textbf{Distillation} \\
SiD ($\alpha=1.2$) ~\cite{Zhou2024SiD} & 1 & 1.71  \\ 
SiD ($\alpha=1$) ~\cite{Zhou2024SiD} & 1 & \textbf{1.63}  \\ \midrule
LMM & 1  &  2.68 \\
LMM & 2  &  \textbf{1.54}  \\ \bottomrule

\end{tabular}
\end{minipage}

\normalsize % Reset to normal font size
\end{table}

